On the Complexity of Reachability in Parametric Markov Decision Processes

This paper studies parametric Markov decision processes (pMDPs), an extension to Markov decision processes (MDPs) where transitions probabilities are described by polynomials over a finite set of parameters. Fixing values for all parameters yields MDPs. In particular, this paper studies the complexity of finding values for these parameters such that the induced MDP satisfies some reachability constraints. We discuss different variants depending on the comparison operator in the constraints and the domain of the parameter values. We improve all known lower bounds for this problem, and notably provide ETR-completeness results for distinct variants of this problem. Furthermore, we provide insights in the functions describing the induced reachability probabilities, and how pMDPs generalise concurrent stochastic reachability games.

==> landscape.tex <==
We now introduce the two families of problems we consider in this work. For the
remaining of this section let us fix a simple pMDP $\mdp$ with parameters
$\Params$, and a set $T$ of target states.

\subsection{Reachability}
The first problem we are interested in is the existence of so-called
\emph{robust parameter values} or lack thereof. More precisely, we ask whether
some instantiation of the $\mdp$ is such that the maximal or minimal probability
of it eventually reaching $T$ compares with $1/2$ in some desired way. In
symbols, for all $\quant_1,\quant_2 \in \{\exists,\forall\}$ and 
$\mathrm{\bowtie} \in
\{\leq, <, >, \geq\}$ we set
\[
  \quant_1\quant_2\reach^{\bowtie} \stackrel{\mathrm{def}}{\iff}
  \quant_1 \inst \in \ParamSpace^{\mathrm{wd}},
  \quant_2 \sched \in \Sched.\;
    \Pr_{\mdp[\Params]}^\sched(\lozenge T) \bowtie \frac{1}{2}.
\]
We write $\quant_1\quant_2\reach^{\bowtie}_{\mathrm{gp}}$ for the version of the
problem where the quantification over instantiations is only over
graph-preserving ones. Furthermore, if $\mdp$ is a pMC we omit the second
quantifier in the notation, e.g. $\exists \reach^{<}$.

\todo[inline]{G: All upper bounds seem to hold for general pMDPs, is this
  correct? If so, we should define the above problems for general pMDPs and
state only the lower bounds for simple pMDPs}
\todo[inline]{G: put one table here, and reference it in the text}

\begin{remark}
	\label{rem:fixedlambda}
	We may restrict ourselves to the fixed threshold $\lambda = 1/2$. Notice that an arbitrary threshold $0 < \lambda' < 1$ is reducible to $1/2$ by the following construction: If $\lambda' \leq 1/2$, we prepend a transition with probability $p := 2\lambda'$ to the initial state and with probability $1-p$ to a sink state.
	Otherwise, if $\lambda' > 1/2$, we prepend a transition with probability $q := 2(1-\lambda')$ to the initial state and $1-q$ to the target state. We will exploit this argument several times. The constructions are depicted in Fig. ??.
\end{remark}
%\paragraph*{Formal definitions of the decision problem}
%\todo[inline]{G: we need to further separate this into subsubsections for upper
%and lower bounds I think}
%
%\begin{definition}
%Let $\mdp$ be a simple pMDP with parameters $\Params$, and $T$ a set of target states.
% We consider the decision problems
%\[ \mathcal{QU}_1 \mathcal{QU}_2 \Pr_{\mdp[\vec{p}]}^\sched(\lozenge T) \sim \frac{1}{2} \]
%with  $\sim \in \{ >, \geq, <, \leq \}$ , $\mathcal{QU}_1\mathcal{QU}_2 \in$  \[\{ \exists \inst \in \ParamSpace^{*}_{\mdp} \exists \sched \in \Sched, 
%	\forall \inst \in \ParamSpace^{*}_{\mdp} \forall \sched \in \Sched, 
%	\exists \inst \in \ParamSpace^{*}_{\mdp} \forall \sched \in \Sched, 
%	\exists \sched \in \Sched \forall \inst \in \ParamSpace^{*}_{\mdp},
%	\forall \sched \in \Sched \exists \inst \in \ParamSpace^{*}_{\mdp} \}, 
% \]
%and $^{*} \in \{ \text{gp,wd} \}$.  
%\end{definition}
%In the remainder, we use the following short-hand notation, e.g. we write $\exists\ParamSpace^{\text{gp}}_{\mdp} \exists \Sched/{>}$ to denote the decision problem whether for a given pMDP $\mdp$: $\exists \inst \in \ParamSpace^{\text{gp}}_{\mdp} \exists \sched \in \Sched\; \Pr_{\mdp[\vec{p}]}^\sched(\lozenge T) > \frac{1}{2}$.
%To indicate that we consider the problem where the input is in fact a pMC, we write, e.g., $\exists\ParamSpace^{\text{gp}}_{\mdp}\text{mc}/{>}$ (and we do not need to quantify over schedulers).
%\todo{G: Wow this notation is heavy :)}
\paragraph*{Considerations for the comparison relations}
In Table~\ref{} we focus on the $\{\geq,>\}$ relations.
The following two lemmas give a justification. 

First, the versions of the problem which use the $\{\leq,<\}$ comparison
relations are polynomial-time interreducible with versions of it using only
$\{>,\geq\}$.
\todo{SJ: What about the version where we first quantify over the strategy? G:
That should not be in the same table anyways}
\begin{lemma} \label{lem:restrict}
  For all $\quant_1\quant_2 \in \{\exists,\forall\}$
  there are polynomial-time many-one reductions
  \begin{itemize}
    \item among the problems $\quant_1 \quant_2 \reach^{>}_{\mathrm{gp}}$ and
      $\quant_1 \quant_2 \reach^{<}_{\mathrm{gp}}$; and
    \item among the problems $\quant_1 \quant_2 \reach^{\geq}_{\mathrm{gp}}$ and
      $\quant_1 \quant_2 \reach^{\leq}_{\mathrm{gp}}$
  \end{itemize}
\end{lemma}
\begin{proof}
  We prove only the first item for arbitrary $\quant_1$ and
  $\quant_2 = \exists$. All other cases
  can be proven analogously.

  First, we deduce from \cite[Thm.~10.122 and Thm.~10.127]{BK08} that in
  polynomial time, and without regarding the actual transition probabilities, we
  can compute from $\mdp$ and a target set $T$ a target set\footnote{Which is some
  adequate union of particular maximal end components}  $T'$ such that 
  \begin{equation}\label{eq:maxeqmininv}
    \max_{\sched \in \Sched} \Pr_{\mdp}^\sched(\lozenge T) = 1 - \min_{\sched
    \in \Sched} \Pr_{\mdp}^\sched(\lozenge T').
  \end{equation}
  And combine this to obtain
  \begin{align*}
    \quant_1 \inst \in \ParamSpace^{\mathrm{gp}},
    \exists \sched \in \Sched.\;
    \Pr_{\mdp[\Params]}^\sched(\lozenge T) > \frac{1}{2}
    & \iff 
    \quant_1 \inst \in \ParamSpace^{\mathrm{gp}}.\;
    \max_{\sched \in \Sched}
    \Pr_{\mdp[\Params]}^\sched(\lozenge T) > \frac{1}{2}\\
    %
    & \overset{\eqref{eq:maxeqmininv}}{\iff}
    \quant_1 \inst \in \ParamSpace^{\mathrm{gp}}.\;
    \left(1 - \min_{\sched \in \Sched}
          \Pr_{\mdp[\Params]}^\sched(\lozenge T')\right) > \frac{1}{2}\\
    %
    & \iff
    \quant_1 \inst \in \ParamSpace^{\mathrm{gp}}.\;
    \min_{\sched \in \Sched} 
    \Pr_{\mdp[\Params]}^\sched(\lozenge T') < \frac{1}{2}\\
    %
    & \iff
    \quant_1 \inst \in \ParamSpace^{\mathrm{gp}},
    \exists \sched \in \Sched.\;
    \Pr_{\mdp[\Params]}^\sched(\lozenge T') < \frac{1}{2}.
  \end{align*}
\end{proof}
We observe that the construction does not work for instantiations that are not
graph-preserving.


\begin{lemma}
  TODO?
\end{lemma}



\subsection{Robust reachability}
The second problem we consider focuses on the schedulers instead of the
parameter values. Mathematically, this means the order of the quantifiers is
swapped from that in the $\quant_1 \quant_2 \reach$ problem. Intuitively, we ask
whether some scheduler gives guarantees on the maximal or minimal probability of
all instantiations of the pMDP eventually reaching $T$. (Thus, it is sometimes
referred to as the \emph{robust scheduler} problem in the literature.)
More formally, for all $\quant_1,\quant_2 \in \{\exists,\forall\}$ and
$\mathrm{\bowtie} \in
\{\leq, <, >, \geq\}$ we set
\[
  \quant_1\quant_2\robreach^{\bowtie} \stackrel{\mathrm{def}}{\iff}
  \quant_2 \sched \in \Sigma,\quant_1 \inst \in \ParamSpace^{\mathrm{wd}}.\;
    \Pr_{\mdp[\Params]}^\sched(\lozenge T) \bowtie \frac{1}{2}.
\]
We adopt the same conventions as for the $\quant_1\quant_2\reach$ problem when
considering graph-preserving instantiations. (Note that the pMC version of the
above problem coincides with the pMC version of the $\quant_1 \quant_2
\reach^{\bowtie}$ problem. We will therefore only use that notation.) Remark \ref{rem:fixedlambda} also applies to the robust reachability problems.


\todo[inline]{G: put the other table here}




\paragraph*{Considerations for the comparison-relation}
In Table~\ref{},\todo{G: the tables should probably be here, after introducing
the notation for the problems} we omitted the different comparison relations, and instead
restricted ourselves to $\geq$.
The following two lemmas give a justification.
\sj{What about the version where we first quantify over the strategy}\todo{G:
  this should work if the quantifiers are the same, otherwise the internal part
will be a $\max \inf$ or $\min \sup$ and then the argument won't work as is}
\begin{lemma}[Restrict to $\geq,>$]
	\label{lem:restrict}
	$\mathcal{Q}_1\ParamSpace^{\text{gp}}_{\mdp} \mathcal{Q}_2 \Sched/{>} \equiv_p \mathcal{Q}_1\ParamSpace^{\text{gp}}_{\mdp} \mathcal{Q}_2 \Sched/{<}  $
	 and 
	 $\mathcal{Q}_1\ParamSpace^{\text{gp}}_{\mdp} \mathcal{Q}_2 \Sched/{\geq} \equiv_p \mathcal{Q}_1 \ParamSpace^{\text{gp}}_{\mdp} \mathcal{Q}_2 \Sched/{\leq}  $
\end{lemma}
\begin{proof}
We prove $\mathcal{Q}_1\ParamSpace^{\text{gp}}_{\mdp} \exists \Sched/{>} \equiv_p \mathcal{Q}_1\ParamSpace^{\text{gp}}_{\mdp} \exists \Sched/{<}  $, the other cases can be proven analogously.

First, we deduce from \cite[Thm.~10.122 and Thm.~10.127]{BK08} that in polynomial time, and without regarding the actual transition probabilities, we can compute from $\mdp$ and a target set $T$ a target set\footnote{Which is some adequate union of particular maximal end components}  $T'$ such that 
\begin{align}\
	\label{eq:maxeqmininv}
	\max_{\sched \in \Sched}\; Pr_{\mdp}^\sigma(\lozenge T) = 1 - \min_{\sched \in \Sched}\; Pr_{\mdp}^\sigma(\lozenge T').
\end{align}
And combine this to obtain
\begin{align*}
	\mathcal{Q}_1 \inst \in \ParamSpace^{\text{gp}}_{\mdp} \exists \sched \in \Sched\; \Pr_{\mdp[\vec{p}]}^\sigma(\lozenge T) > \frac{1}{2}
	& \iff 
	\mathcal{Q}_1 \inst \in \ParamSpace^{\text{gp}}_{\mdp} \max_{\sched \in \Sched}\; \Pr_{\mdp[\vec{p}]}^\sigma(\lozenge T) > \frac{1}{2}\\
	& \overset{\eqref{eq:maxeqmininv}}{\iff}
	\mathcal{Q}_1 \inst \in \ParamSpace^{\text{gp}}_{\mdp} 1{-}\min_{\sched \in \Sched}\; \Pr_{\mdp[\vec{p}]}^\sigma(\lozenge T') > \frac{1}{2}\\
	& \overset{}{\iff}
	\mathcal{Q}_1 \inst \in \ParamSpace^{\text{gp}}_{\mdp} \min_{\sched \in \Sched}\; \Pr_{\mdp[\vec{p}]}^\sigma(\lozenge T') < \frac{1}{2} \\
	& \overset{}{\iff}
	\mathcal{Q}_1 \inst \in \ParamSpace^{\text{gp}}_{\mdp}  \exists {\sched \in \Sched}\; \Pr_{\mdp[\vec{p}]}^\sigma(\lozenge T') < \frac{1}{2}
\end{align*}

\end{proof}

\begin{lemma}[Restrict to $\geq$, robust strategy version]
	\label{lem:restrict2}
	$\mathcal{Q}_1 \Sched\mathcal{Q}_2 \ParamSpace^{\text{gp}}_{\mdp}/{\geq} \equiv_p \mathcal{Q}_1 \Sched\mathcal{Q}_2 \ParamSpace^{\text{gp}}_{\mdp}/{\leq}$
\end{lemma}
\begin{proof}
Similar to \eqref{eq:maxeqmininv}, we have
	\begin{align}\
	\max_{\sched \in \Sched} \inf_{\inst \in \ParamSpace^{\text{gp}}}\; Pr_{\mdp[\inst]}^\sigma(\lozenge T) = 1 - \min_{\sched \in \Sched}\sup_{\inst \in \ParamSpace^{\text{gp}}}\; Pr_{\mdp[\inst]}^\sigma(\lozenge T').
\end{align}
\end{proof}


We observe that the construction does not work for instantiations that are not graph-preserving.



\subsection{Fixed Parameters}



\begin{remark}
Lack of graph-preservation is not an issue here. 
For a fixed number of parameters, the number of of graph-preserving regions is constant. 
A more complete construction is given in \cite{prophesy_journal}.\todo{G: this
  should be more precise; I guess what we want to say is that we can consider a
  constant number of pMDPs (with graph-preserving valuations) obtained by choosing valuations so as to change
topology\ldots is this for general pMDPs or only for simple ones?}
\end{remark}

\begin{lemma}[Fixed parameters, $\exists\ParamSpace^{\text{*}}_{\mdp} \exists
  \Sched/\unrhd$ in NP]\todo{G: the $\unrhd$ notation was not introduced}
\label{lem:fp-epes-np}
	
\end{lemma}
\begin{proof}
Reformulate as $\exists \Sched \exists\ParamSpace^{\text{*}}_{\mdp}/\unrhd$.
Guess the memoryless scheduler. 
Construct the induced pMC, and verify in P.
\end{proof}

In the non-parametric case, a scheduler $\sigma$ for an MDP $\mdp$ is called \emph{minimal} if it minimizes $Pr_{\mdp}(\lozenge T)$ in the induced MC , i.e. if
$\sigma = arg\min_{\sched' \in \Sched}\; Pr_{\mdp}^{\sigma'}(\lozenge T).$
Consider the probabilities $x_s = Pr_{\mdp}^{\sigma}(s \rightarrow \lozenge T)$ for $s \in S$.
It is well-known (\tw{reference and check if this is actually correct}) that $\sigma$ is minimal if and only if
\begin{align*}
	x_s \leq \sum_{s' \in S}P(s,\alpha,s')x_{s'}
\end{align*}
holds for all $s \in S$ and all $\alpha \in \Act$. (There is a similar condition for \emph{maximal} schedulers.) The minimality criterion may also be lifted to the case of a parametric $\mdp$: Let $f_s(\inst) = Pr_{\mdp}^{\sigma}(s \rightarrow \lozenge T)$ be the the reachability probability from $s$ to $T$ as a rational function of the (graph-preserving) parameters of $\mdp$. Then $\sigma$ is minimal \emph{everywhere} on the parameter space $\ParamSpace^{\text{gp}}_{\mdp}$ if and only if 
\begin{align*}
	f_s(\inst) \leq \sum_{s' \in S}P(s,\alpha,s')f_{s'}(\inst)
\end{align*}
holds for all $\inst \in \ParamSpace^{\text{gp}}_{\mdp}$, $s \in S$ and $\alpha \in \Act$. The negation of this condition can be reformulated as the ETR formula
\begin{align}
	\label{eq:optimalstratparametric}
	\exists \inst: \neg\big(\Phi_{\text{gp}}(\inst) \rightarrow \bigwedge_{s \in S} \bigwedge_{\alpha \in \Act} g_s(\inst) \prod_{s' \neq s}h_{s'}(\inst) \leq \sum_{s' \in S}P(s, \alpha, s')g_{s'}(\inst)\prod_{s'' \neq s'}h_{s''}(\inst) \big)
\end{align}
where $\Phi_{\text{gp}}(\inst)$ is a formula which is true if and only if $\inst$ is graph-preserving and $f_s =: \frac{g_s}{h_s}$ for polynomials $g_s$, $h_s$. This motivates the next lemma:

\begin{lemma}
	\label{lem:checkstrategyinp}
	In the fixed parameter case, checking whether a given strategy is everywhere (resp. somewhere) minimal (resp. maximal) on the graph-preserving parameter space is in P.
\end{lemma}
\begin{proof}
	Computing the rational functions $f_s = \frac{g_s}{h_s}$ is in P. For everywhere minimal strategies, formula (\ref{eq:optimalstratparametric}) is of polynomial size, has only a fixed number of variables and can therefore be checked in polynomial time. For the other three cases, formulas similar to (\ref{eq:optimalstratparametric}) can be constructed.
\end{proof}

\begin{theorem}[Fixed parameters, $\exists\ParamSpace^{\text{*}}_{\mdp} \forall \Sched/\unrhd$ in NP]
	
\end{theorem}
\begin{proof}
\sj{This proof should be extended a bit}

	Reformulate as $\exists p \min$.
	Guess a minimal (memoryless)  scheduler.
	Use Lemma \ref{lem:checkstrategyinp}.

\end{proof}


\begin{theorem}[Fixed parameters, $\exists \Sched \forall\ParamSpace^{\text{*}}_{\mdp}/?$ NP-complete]
	
\end{theorem}

\begin{proof}
Membership in NP is analogous to Lemma~\ref{lem:fp-epes-np}. 
NP-hardness is based on a reduction from 3-SAT, and requires a single parameter only. Details can be found in Appendix~\ref{App:fp-esfp-np}.	
\end{proof}


\begin{remark}
In general, optimal robust strategies do require
memory~\cite{DBLP:journals/corr/ArmingBS17} and randomisation (via a similar
construction).\todo{G: this should go earlier, and we should motivate our
  restriction to memoryless strategies; what do we know about general
strategies?}
\end{remark}



\subsection{Arbitrary Parameters}

\paragraph*{Revisiting Markov Chains}

The following lemma reformulates~\cite[Theorem 5]{DBLP:conf/uai/Junges0WQWK018}.
\begin{lemma}
\label{lem:existwdgeeqexistgpge}
$\exists\ParamSpace^{\text{wd}}_{\mdp}\text{mc}/{>}$  $\leq_p$ $\exists\ParamSpace^{\text{gp}}_{\mdp}\text{mc}/{>}$.
\end{lemma}
\begin{proof}
	For this reduction, we do not need to adapt the pMC or the considered property.
	Moreover, as graph-preserving instantiations are a special case of well-defined instantiations, we only need to consider the absence of a graph-preserving instantiation, and argue that then, there is also no well-defined instantiation.


	Let $S^u_{=0} = \{  | \}$ denote states that reach the target with probability zero in instantiation $u$.
	Let $S^\text{gp}_{=0} = \{  | \}$ denote states that reach the target with probability zero for any graph-preserving instantiation.
	Then $S^\text{gp}_{=0} \subseteq S^u_{=0}$.
	
	Consider a well-defined, non-graph preserving instantiation $u$.
	\sj{Pretty annoying to formalise}
	\begin{itemize}
	\item 
	Either $S^\text{gp}_{=0} = S^u_{=0}$: 
	Then, the characterising linear equation systems coincide, they have the same solution $\sol_\mdp$ and thus the probability at $u$ is given by $\sol_\mdp(u)$.
	As $\sol_\mdp$ is continuous on $\{ u \in \ParamSpace^{\text{wd}} \mid S^u_{=0} =S^\text{gp}_{=0} \}$~\cite{DBLP:conf/atva/QuatmannD0JK16}, if $\sol_\mdp(u) > \frac{1}{2}$, then there also exist a graph-preserving $u'$ such that $\sol_\mdp(u') > \frac{1}{2}$, which contradicts our assumption.
	
	\item
	Otherwise $S^\text{gp}_{=0} \subset S^u_{=0}$:
	\sj{Finish this}
	\end{itemize}

	
	\sj{What kind of assumptions do we need on the shape of the graph-preserving region}
	
\end{proof}
We can show that assuming graph-preservation is not harder than assuming well-definedness for lower-bounded properties.
\begin{lemma}
\label{lem:gpiseasier}
	$\exists\ParamSpace^{\text{gp}}_{\mdp}\text{mc}/{\unrhd}$  $\leq_p$ $\exists\ParamSpace^{\text{wd}}_{\mdp}\text{mc}/{\unrhd}$. 
	%and analogously $\forall\ParamSpace^{\text{gp}}_{\mdp}\text{mc}/{\unlhd}$  $\leq_p$ $\forall\ParamSpace^{\text{wd}}_{\mdp}\text{mc}/{\unlhd}$
\end{lemma}
\sj{What about other relations here}
\begin{proof}
Given a simple pMC $\mdp$. We extend the pMC with a gadget outlined in Fig.~\ref{fig:lemgpiseasier}. Formally, we construct an pMC $\mdp'$ with with states $S'=S \cup \{ s_p, s'_p \mid p \in \Params \}$, initial state $s_{\Params_1}$ and \[ P'(s,s') = \begin{cases}
 P(s,s) & \text{if }s,s' \in S \\
 p    & \text{if }s = s' = s_p \\
 1{-}p & \text{if }s = s' = s'_p \\
 1{-}p & \text{if }s = s_p \text{ and } s' = s'_p \\
 p & \text{if }s = s'_p \text{ and } s' = \text{next}(s'_{p}) \\
 0 & \text{otherwise.}	
 \end{cases}
 \]
where $\text{next}(s'_p)$ is $s_q$ if $p = \Params_i$ and $q = \Params_{i+1}$ for some $i < |\Params|$, and $\sinit$ if $i = \Params$.
The pMC $\mdp'$ is only linearly larger than $\mdp$. Observe that the construction of the gadget can be adapted for non-simple pMCs.
By construction \[ \Pr_{\mdp'[\inst]}(\lozenge T) = \Pr_{\mdp[\inst]}(\lozenge T) \cdot \Pr_{\mdp'[\inst]}(\lozenge \{ \sinit \}). \]
We observe the following: \begin{align}& \forall \inst \in \ParamSpace^\text{gp}~ \Pr_{\mdp'[\inst]}(\lozenge \{ \sinit \}) = 1 \text{ and thus } \Pr_{\mdp'[\inst]}(\lozenge T) = \Pr_{\mdp[\inst]}(\lozenge T)\text{, and}\label{eq:lemgpiseasier:obs1} \\
& \forall \inst \in \ParamSpace^\text{gp} \setminus \ParamSpace^\text{wd} \Pr_{\mdp'[\inst]}(\lozenge \{ \sinit \}) = 0\label{eq:lemgpiseasier:obs2}
\end{align}

\noindent We have:
\begin{align*}
	\exists\ParamSpace^{\text{gp}}_{\mdp} \Pr_{\mdp[\inst]}(\lozenge T) {\unrhd} \lambda
	\implies 
	\exists\ParamSpace^{\text{gp}}_{\mdp'} \Pr_{\mdp'[\inst]}(\lozenge T) {\unrhd} \lambda 
	\overset{\eqref{eq:lemgpiseasier:obs1}}{\implies}
	\exists\ParamSpace^{\text{wd}}_{\mdp'} \Pr_{\mdp'[\inst]}(\lozenge T) {\unrhd} \lambda
\end{align*}
and
\begin{align*}
	\not\exists\ParamSpace^{\text{gp}}_{\mdp} \Pr_{\mdp[\inst]}(\lozenge T) {\unrhd} \lambda 
	\implies 
	\forall\ParamSpace^{\text{gp}}_{\mdp} \Pr_{\mdp[\inst]}(\lozenge T) {\unlhd} \lambda 
	\overset{\eqref{eq:lemgpiseasier:obs2}}{\implies}
	\forall\ParamSpace^{\text{wd}}_{\mdp} \Pr_{\mdp[\inst]}(\lozenge T) {\unlhd} \lambda 
	\implies
	\not\exists\ParamSpace^{\text{wd}}_{\mdp} \Pr_{\mdp[\inst]}(\lozenge T) {\unrhd} \lambda 
\end{align*}


\end{proof}
\begin{figure}
\begin{tikzpicture}[initial text=]
	\node[initial,state] (s1) {$s_{\Params_1}$};
	\node[state, right=of s1] (s2) {$s'_{\Params_1}$};
	\node[state, draw, right=of s2] (s3) {$s_{\Params_2}$};
	\node[state, right=of s3] (s4) {$s'_{\Params_2}$};
	\node[circle, right=of s4] (s5) {$\hdots$};
	\node[state, right=of s5] (s6) {$s'_{\Params_n}$};
	\node[state, right=of s6] (s7) {$\sinit$};
	
	\draw[->] (s1) edge node[auto] {$1{-}p_1$} (s2);
	\draw[->] (s2) edge node[auto] {$p_1$} (s3);
	\draw[->] (s3) edge node[auto] {$1{-}p_2$} (s4);
	%\draw[->] (s4) edge node {$p_2$} (s2);
	\draw[->] (s6) edge node[auto] {$p_n$} (s7);

	\draw[->] (s1) edge[loop above] node[auto] {$p_1$} (s1);
	\draw[->] (s2) edge[loop above] node[auto] {$1{-}p_1$} (s2);
	\draw[->] (s3) edge[loop above] node[auto] {$p_2$} (s3);
	\draw[->] (s6) edge[loop above] node[auto] {$1{-}p_n$} (s6);
	
\end{tikzpicture}	
\caption{Gadget for the proof of Lemma~\ref{lem:gpiseasier}}
\label{fig:lemgpiseasier}
\end{figure}
%%
An immediate consequence is the following equivalence:
\begin{corollary}
	\label{cor:gpvswdequiv}
	$\exists\ParamSpace^{\text{gp}}_{\mdp}\text{mc}/{>}$  $\equiv_p$ $\exists\ParamSpace^{\text{wd}}_{\mdp}\text{mc}/{>}$.
\end{corollary}
The following is a simple corollary to \cite[Thm.~3]{DBLP:journals/corr/Chonev17}. %for $\geq 1$ relation.

\begin{lemma}
\label{lem:epwdgeqnphard}
	$\exists\ParamSpace^{\text{wd}}_{\mdp}\text{mc}/{\geq}$ is NP-hard.
\end{lemma}
\begin{proof}
\begin{itemize}
	\item The decision problem $\exists\ParamSpace^{\text{wd}}_{\mdp} \Pr_{\mdp[\vec{p}]}(\lozenge T) \geq 1$ is NP-complete~\cite[Thm.~3]{DBLP:journals/corr/Chonev17}.
	\item Trivially, $\exists\ParamSpace^{\text{wd}}_{\mdp} \Pr_{\mdp[\vec{p}]}(\lozenge T) \geq 1\quad \leq_p \quad \exists\ParamSpace^{\text{wd}}_{\mdp'} \Pr_{\mdp[\vec{p}]}(\lozenge T) \geq \frac{1}{2}$.
	\end{itemize}

\end{proof}

 
\begin{theorem}
	\label{thm:chonevextended}
	$\exists\ParamSpace^{\text{wd}}_{\mdp}\text{mc}/{>}$ is NP-hard.
\end{theorem}
\begin{proof}

  We extend the proof of Thm. 3 from \cite{DBLP:journals/corr/Chonev17} and show that the same 3SAT-reduction also applies to our $\exists\ParamSpace^{\text{wd}}_{\mdp}\text{mc}/{>}$ problem. We first reformulate the construction in our notation, sticking to Chonev's notation whenever possible:
	
	Let $\phi = \phi_1 \wedge ... \wedge \phi_k$ be a given 3SAT-formula, i.e. the $\phi_j$ are of the form
	$$\phi_i = l_{j,1} \vee l_{j,2} \vee l_{j,3},$$
	where the $l_{i,j}$ are \emph{literals} (variables or negated variables). Let $x_1, ..., x_m$ be the variables of $\phi$. The pMC $\mdp_\phi = (S, \vec{p}, \sinit, P)$ is defined as follows:
	\begin{itemize}
		\item $S =
			\{x_i, \overline{x_i} \mid 1 \leq i \leq m\} \cup
		    \{\phi_i \mid 1 \leq i \leq k\} \cup
		    \{v_i \mid 0 \leq i \leq m\} \cup
		    \{F, T\}$ are the $3m + k + 3$ states, $F$ and $T$ indicate failure and success,
		\item $\vec{p} = (p_1, ..., p_m, q_{1,1}, q_{1,2}, q_{1,3}, ..., q_{k,1}, q_{k,2}, q_{k,3})$ are the parameters,
		\item $\sinit = v_0$ is the initial state,
		\item for all $1 \leq i \leq m$ and $1 \leq j \leq k$ we define the transition probabilities as\\
		\begin{alignat*}{2}
			&P(v_{i-1}, x_i) = p_i, &\quad &P(v_{i-1}, \overline{x_i}) = 1-p_i, \\
			&P(x_i, v_i) = p_i, && P(\overline{x_i}, v_i) = 1-p_i, \\
			&P(x_i, F) = 1-p_i, && P(\overline{x_i}, F) = p_i, \\
			&P(v_m, \phi_j) = \frac{1}{k+1}, && P(v_m, T) = \frac{1}{k+1}, \\
			&P(\phi_j, l_{j,t}) = q_{j,t}, && t \in \{1,2,3\}.
		\end{alignat*}
	\end{itemize}
	Moreover, we let $P(s,t) = 0$ for each pair $(s,t)$ of states not specified above. The construction is depicted in \ref{fig:chonevgadget}.
	
	\textbf{Auxiliary Claim:} If $\phi$ is unsat, then for all well-defined valuations $u$ there exists some clause $\phi_{j^*}$, $1 \leq j^* \leq k$, such that $P(l_{j^*,t}, F)[u] \geq \frac{1}{2}$ for all $t\in\{1,2,3\}$.
	
	\emph{Proof of the auxiliary claim:} Let $\phi$ be unsat and fix any parameter valuation $u$. 
	Suppose for contradiction that for every clause $\phi_j$ there is a `witness' literal $l_{j,t}$ such that $P(l_{j,t}, F)[u] < \frac{1}{2}$.
	
	
	Then by construction it holds that either
	\begin{enumerate}
		\item $l_{j,t}$ is a variable $x_i$ and $u(p_i) > \frac{1}{2}$,
		\item $l_{j,t}$ is a negated variable $\overline{x_i}$ and $u(p_i) < \frac{1}{2}$.
	\end{enumerate}
	
	We consider a variable assignment $\mathcal{I}_u$ for $\phi$ as follows:
	$$\mathcal{I}_u(x_i) =
	\begin{cases}
		1, & \text{if } u(p_i) > \frac{1}{2}, \\
		0, & \text{if } u(p_i) < \frac{1}{2}, \\
		\text{arbitrary}, & \text{if } u(p_i) = \frac{1}{2}.
	\end{cases}$$
	In both of the two cases, $\mathcal{I}$ satisfies clause $\phi_j$. 
	Thus $\phi$ is sat, contradiction.

	\textbf{Claim:}	If $\phi$ is unsat, then $\Pr_{\mdp_\phi[\vec{p}]}(\lozenge T) \leq \frac{2}{3}$ for all parameter valuations $\vec{p}$.
	
	\emph{Proof of the claim:} 
	\newcommand{\prfromto}[2]{Pr(#1 \rightarrow #2)}
	Once again let $\phi$ be unsat and fix a parameter valuation $\vec{p}$. We denote by $\prfromto{s}{t}$ the probability to move from state $s$ to $t$ in $\mdp_\phi[\vec{p}]$.
	Let $j^*$ be like in the previous claim. We have
	$$\prfromto{\phi_{j^*}}{v_m} = \sum_{t=1}^3 q_{j^*, t}\prfromto{l_{j^*,t}}{v_m} \leq \frac{1}{2}\sum_{t=1}^3 q_{j^*, t} = \frac{1}{2}.$$
	Consequently, for $\prfromto{v_m}{v_m}$ it holds that
	\begin{align*}
		\prfromto{v_m}{v_m} &= \sum_{j \neq j^*}\prfromto{v_m}{\phi_j}\prfromto{\phi_j}{v_m} + \prfromto{v_m}{\phi_{j^*}}\prfromto{\phi_{j^*}}{v_m} \\
		& \leq \frac{k-1}{k+1} + \frac{1}{2(k+1)} = \frac{2k-1}{2(k+1)}
	\end{align*}
	From the equation
	$$\prfromto{v_m}{T} = \frac{1}{k+1} + \prfromto{v_m}{v_m}\prfromto{v_m}{T}$$
	we therefore obtain the estimate
	$$\prfromto{v_m}{T} \leq \frac{2}{3}.$$
	by a straightforward calculation. Noticing that 
	$$\Pr_{\mdp_\phi[\vec{p}]}(\lozenge T) = \prfromto{\sinit}{T} = \prfromto{\sinit}{v_m}\prfromto{v_m}{T} \leq \prfromto{v_m}{T}$$
	completes the proof.
	
	Together with Chonev's argument for '$\Longrightarrow$' we now have
	$$\phi \text{ is satisfiable } \Longleftrightarrow \exists \vec{p} \Pr_{\mdp_\phi[\vec{p}]}(\lozenge T) > \frac{2}{3}$$
	and the claim follows.
\end{proof}

\begin{figure}
	\label{fig:chonevgadget}
	\centering
	\includegraphics[scale=0.4]{figures/chonev-reduction}
	\caption{Chonev's construction used in the proof of Thm. \ref{thm:chonevextended} (the failure state $F$ is duplicated)}
\end{figure}

\begin{corollary}
	$\exists\ParamSpace^{\text{gp}}_{\mdp}\text{mc}/{>}$ and $\exists\ParamSpace^{\text{gp}}_{\mdp}\text{mc}/{<}$ are NP-hard.
\end{corollary}
\begin{proof}
Lemma \ref{lem:existwdgeeqexistgpge}, Theorem \ref{thm:chonevextended} and Lemma \ref{lem:restrict}.
\end{proof}

\paragraph*{MDPs}
 
\subparagraph*{Concurrent stochastic reachability games}
A \emph{Concurrent Stochastic Reachability Game} (CSRG) is a two player game $\csrg$ played on a finite set $S$ of states. The objective of player I (\emph{reachability} player) is to reach a set $T \subseteq S$ of target stets while player II (\emph{safety player}) seeks to avoid that any state in $T$ is ever reached.

A play of $\csrg$ begins in an initial state $\csrginit$ and proceeds as follows: In state $s$, both players $i \in \{\text{I}, \text{II}\}$ \emph{concurrently} select an action $\csrgactioni{} \in A_s^i$, the finite set of actions available to player $i$ in state $s$. The game then picks a successor state $s'$ according to a fixed observable probability distribution $P_{s,\csrgactionI{}, \csrgactionII{}}$ over the state space $S$ and the play continues in $s'$. The transitioning from $s$ to $s'$ is called a \emph{round} of $\csrg$.

Player I wins $\csrg$ as soon as a state in $T$ is reached. If this is not the case after a finite number of rounds, then player II wins.

A \emph{strategy} $\sigma^i$ for player $i$ is a rule that associates a given history \[
\csrginit = s_0 \overset{\csrgactionI{0}, \csrgactionII{0}}{\longrightarrow} s_1\ \dots\ s_{k-1} \overset{\csrgactionI{k-1},\csrgactionII{k-1}}{\longrightarrow} s_k
\]

of played rounds to a probability distribution over the actions $A_{s_k}^i$ available in the current state $s_k$. The set of all strategies for player $i$ is denoted by $\Sigma^i$.

We call $\sigma^i$ a \emph{stationary} strategy if it does no depend on the history, i.e. $\sigma^i$ can be viewed as a mapping that defines a fixed probability distribution $\sigma^i_s$ over $A_s^i$ for each state $s \in S$.

The \emph{instantiation} $\csrg[\sigma^i]$ of $\csrg$ with a stationary strategy for player $i$ is the structure obtained by forcing player $i$ to follow $\sigma^i$. Notice that $\csrg[\sigma^i]$ is an MDP. Conversely, every MDP may be viewed as a CSRG where $|A^i_s| = 1$ for one of the players $i$ and all $s \in S$.

We let $\Pr_\csrg^{\csrgstratI, \csrgstratII}(\lozenge T)$ be the probability that $T$ is reached if both players $i$ follows the strategies $\sigma^i$. The player-I-value (player-II-value , resp.) is defined as \[
val_{\text{I}}(\csrg) = \sup_{\csrgstratI \in \Sigma^\text{I}}\inf_{\csrgstratII \in \Sigma^\text{II}}\Pr_\csrg^{\csrgstratI, \csrgstratII}(\lozenge T),\ \ \ val_{\text{II}}(\csrg) = 1 - \inf_{\csrgstratII \in \Sigma^\text{II}}\sup_{\csrgstratI \in \Sigma^\text{I}}\Pr_\csrg^{\csrgstratI, \csrgstratII}(\lozenge T)
\]
i.e. $val_i(\csrg)$ is the maximal winning probability of player $i$ that can be guaranteed against all strategies of the other player.

\begin{theorem}[CSRG properties]
	\label{thm:csrgprops}
	The following two statements hold:
	\begin{enumerate}
		\item $val_{\text{I}}(\csrg) + val_{\text{II}}(\csrg) = 1$ (CSRGs are determined)
		\item $val_{\text{II}}(\csrg) = \Pr_\csrg^{\csrgstratI, \csrgstratII}(\lozenge T)$ for a stationary strategy $\csrgstratII$ and a deterministic stationary strategy $\sigma^I$.
	\end{enumerate}
\end{theorem}

The existence of stationary optimal strategies allows us to encode a CSRG in a pMDP as we will show next.

\begin{definition}[Decision problem \texttt{CSRG}]
The problem \texttt{CSRG} is defined as:
Given $\csrg$ and a rational threshold $\lambda \in (0,1)$, does $val_\text{I}(\csrg) \sim \lambda$ hold?
\end{definition}

\begin{theorem}
\label{thm:csrghardness}
	$\emph{\texttt{CSRG}} \leq_p \exists\ParamSpace^{\text{wd}}_{\mdp}\forall\Sigma$
\end{theorem}
\begin{proof}
	For a given CSRG $\csrg$ with state space $S_\csrg$ we define a pMDP $\mdp$ as follows:\\
	$\mdp = \pmdptuple$, where
	\begin{itemize}
		\item $S = S_\csrg \cup \{s_{\csrgactionI{}} \mid s \in S_\csrg, \csrgactionI{} \in A^\text{I}_s\} \cup \{s_{\csrgactionI{}, \csrgactionII{}} \mid s \in S_\csrg, \csrgactionI{} \in A^\text{I}_s, \csrgactionII{} \in A^\text{II}_s\}$ 
		\item $\Params = \bigcup_{s \in S_\csrg} A^\text{II}_s$ and $\Act = \bigcup_{s \in S_\csrg} A^\text{I}_s$, where we assume w.l.o.g. that the $A_s^i$ are pairwise disjoint for all $s \in S_\csrg$.
		\item For all $s,s' \in S_\csrg, \csrgactionI{} \in A^\text{I}_s, \csrgactionII{} \in A^\text{II}_s$ we define
		\begin{itemize}
			\item $P(s,\csrgactionI{},s_{\csrgactionI{}}) = 1$,
			\item $P(s_{\csrgactionI{}}, s_{\csrgactionI{}, \csrgactionII{}}) = \csrgactionII{}$,
			\item $P(s_{\csrgactionI{}, \csrgactionII{}}, s') = P_{s,\csrgactionI{}, \csrgactionII{}}(s')$,
		\end{itemize}
		where we omit the actions in states where only one action is available.
	\end{itemize}
	By theorem \ref{thm:csrgprops}, $val_\text{I}(\csrg) \sim \lambda \Leftrightarrow  1 - \lambda \sim val_\text{II}(\csrg)$
	Then $\mdp$ mimics $\csrg$. \ref{thm:csrgprops}
	
	Formally, we show that $val_\text{II}(\csrg) = $
\end{proof}


 

\begin{lemma}
\label{lem:existwdgeeqexistgpge}
$\exists\ParamSpace^{\text{wd}}\exists\Sched/{\unrhd}$  $\equiv_p$ $\exists\ParamSpace^{\text{wd}}\text{mc}/{\unrhd}$.
\end{lemma}
\begin{proof}
	
\end{proof}

\begin{theorem}
	$\exists\ParamSpace^{\text{gp}}\forall\Sched/{\unrhd}$ is NP-hard (even for acyclic pMDPs).
	\end{theorem}
The proof is an adaption of an NP-hardness result for pMCs with 
two reachability objectives~\cite[Theorem 8]{infocomp}. 
The adapted proof is attached in Appendix~\ref{}.

	





